PC-LoRA: Low-Rank Adaptation for Progressive Model Compression with Knowledge Distillation

Low-rank adaption (LoRA) is a prominent method that adds a small number of learnable parameters to the frozen pre-trained weights for parameter-efficient fine-tuning. Prompted by the question, ``Can we make its representation enough with LoRA weights solely at the final phase of finetuning without the pre-trained weights?'' In this work, we introduce Progressive Compression LoRA~(PC-LoRA), which utilizes low-rank adaptation (LoRA) to simultaneously perform model compression and fine-tuning. The PC-LoRA method gradually removes the pre-trained weights during the training process, eventually leaving only the low-rank adapters in the end. Thus, these low-rank adapters replace the whole pre-trained weights, achieving the goals of compression and fine-tuning at the same time. Empirical analysis across various models demonstrates that PC-LoRA achieves parameter and FLOPs compression rates of 94.36%/89.1% for vision models, e.g., ViT-B, and 93.42%/84.2% parameters and FLOPs compressions for language models, e.g., BERT.

==> figure/wds.tex <==
\centering
\includegraphics[width=0.8\linewidth]{figure/wds3.pdf}
\captionof{figure}{Weight Decay Scheduler}
\label{fig:wds}

==> sec/6_ack.tex <==
\section{Acknowledgement}
This research was partly supported by Institute of Information \& communications Technology Planning \& Evaluation (IITP)
grant funded by the Korea government (MSIT) (No. RS2022-00187238, Development of Large Korean Language
Model Technology for Efficient Pre-training).

%and Brian Impact Foundation, a non-profit organization dedicated to the advancement of science and technology for all.

